An Extended Tutorial and Vocabulary for Relational Language Design in an Era of AI-Assisted Query Generation

Relational query languages have been studied and used for more than 50 years, with SQL dominant in practice. Today, queries are increasingly generated by machines and read by humans. At the same time, the landscape also includes dataframe, pipeline, logical, functional, graph, and relational programming notations. These developments invite two related questions beyond expressive power: which relational structures do languages make explicit, and how well can notation support users in reading and revising queries? This 3-hour tutorial extends an earlier SIGMOD'26 tutorial in three directions: recursive and path queries (connecting relational and graph query languages), nested relational data, and relational languages for problems beyond PTIME. Rather than beginning from formal definitions, we start from example queries and compare how different languages express the same intent. To compare recurring structure across notations, we use Abstract Relational Calculus (ARC) and Relational Diagrams as reference representations. From these examples, we develop a vocabulary for relational language design, including information need, query mapping, relational pattern structure, relational pattern denotation, and semantic conventions. Participants will leave with a framework for comparing existing and future relational languages, a precise vocabulary for articulating design trade-offs, and a concrete set of examples connecting classical database languages with alternative proposals.

==> datalabmacros.tex <==

\usepackage{anyfontsize}	%
\usepackage[T1]{fontenc} %




\usepackage[table]{xcolor}

\usepackage{amsthm}
\usepackage{graphicx} %
\usepackage{placeins}
\usepackage{float}
\usepackage{afterpage}
\usepackage{url}
\usepackage{enumitem} %
\usepackage{soul} %
\usepackage{listings} %

\usepackage{tabularx} %
\usepackage{multirow}
\usepackage{hhline} %
\usepackage{diagbox}

\usepackage{booktabs}  %





\usepackage{tikz}
\usetikzlibrary{arrows.meta,fit,backgrounds}
\newif\ifshowqueryrolearrows





\RequirePackage{etoolbox}	%
\newcommand{\iflabelexists}[3]{\ifcsundef{r@#1}{#3}{#2}}























\let\subcaption\relax
\let\subfloat\relax
\usepackage{subcaption}		%
\captionsetup[figure]{
	font=small,%
	aboveskip=3pt,%
	}		
\captionsetup[table]{font+=small}		%
\captionsetup[subfigure]{
	font+=small,%
	}







\usepackage[ruled,noend,linesnumbered]{algorithm2e} %

\DontPrintSemicolon     %
\SetNlSty{}{}{}                %
\SetAlgoInsideSkip{smallskip}   %
\SetAlCapSkip{1.5mm}             %
\setlength{\algomargin}{1.5mm}    %
\SetInd{1.5mm}{1.5mm}             %

\SetAlFnt{\small}			%
\SetAlCapFnt{\small}		%
\SetAlCapNameFnt{\small}





\newtheorem{hypothesis}{Hypothesis}






\newcommand{\todo}[1]{{\color{red}[\textbf{TODO}:{#1}]}} %
\newcommand{\wolf}[1]{{{\color{red}{[\textbf{wg}: #1]}}}} %
\newcommand{\deprecate}[1]{{{\color{gray}{#1}}}} %
\newcommand{\out}[1]{{\color{gray}\textbf{OUT}: #1}}


\newcommand{\later}[1]{{\color{blue}\textbf{LATER}: #1}}
\newcommand{\laterr}[1]{{\color{blue}\textbf{LATERR}: #1}}

\newcommand{\revision}[1]{{\color{blue}{#1}}}



\newcommand{\hide}[1]{} 		%







\newcommand{\mkclean}{
    \renewcommand{\out}[1]{\hide}
    \renewcommand{\todo}{\hide}
    \renewcommand{\deprecate}{\hide}
    \renewcommand{\wolf}[1]{\hide}
}
















\usepackage[capitalise,nameinlink]{cleveref} %

\crefname{algocf}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefalias{AlgoLine}{line}%
\crefname{property}{Property}{Properties}

\crefformat{equation}{(#2#1#3)}						%
\crefrangeformat{equation}{(#3#1#4) to~(#5#2#6)}
\crefmultiformat{equation}{(#2#1#3)}%
{ and~(#2#1#3)}{, (#2#1#3)}{ and~(#2#1#3)}




\newcommand{\eref}[1]{\textup{\ref{#1}}}






\AtEndPreamble{%
    \hypersetup{colorlinks,
      linkcolor=ACMDarkBlue,		%
      citecolor=blue,
      urlcolor=ACMDarkBlue,
      filecolor=ACMDarkBlue,
      pdfcreator = {},
      }}










	
	\usepackage[normalem]{ulem} %
	\newcommand\highl{\bgroup\markoverwith
	  {\textcolor{yellow}{\rule[-.5ex]{2pt}{2.5ex}}}\ULon}





\usepackage{marginnote}
\newcommand{\rebuttal}[2]{\marginnote{\textbf{\textcolor{blue}{#1}}}{\color{blue}#2}}
\newcommand{\new}[1]{{\color{blue}{#1}}}








\usepackage{tcolorbox}		%
\tcbuselibrary{breakable,skins}		%


\tcbset{examplestyle/.style={
	enhanced jigsaw,	%
	colback=gray!10,	%
	colframe=gray!20,	%
	arc=0mm,			%
	boxrule=1pt,		%
	left=1mm,
	right=1mm,
	left skip=0mm,  %
	right skip=0mm, %
	top=1mm,		%
	bottom=1mm,		%
	breakable,		%
	parbox = false,		%
	before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},
	after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
	boxsep = 0mm,					%
	topsep at break=0pt,			%
	bottomsep at break=0pt,			%
	pad at break=0mm,
	pad before break=0mm,		
	pad after break=1mm,		
	bottomrule at break=0mm,
	toprule at break=0mm,		
	}}

\tcolorboxenvironment{example}{examplestyle}



\newtheoremstyle{abcd}%
  {}%
  {}%
  {\upshape}%
  {}%
  {\itshape}%
  {.}%
  {.5em}%
  {}%

\theoremstyle{abcd}
\newtheorem{example}{Example}




\tcbset{theoremstyle/.style={
		enhanced jigsaw,	%
		colback=white,	%
		colframe=black,	%
		arc=0mm,			%
		boxrule=1pt,		%
		left=1mm,
		right=1mm,
		left skip=0mm,  %
		right skip=0mm, %
		top=1mm,		%
		bottom=1mm,		%
		breakable,		%
		parbox = false,		%
		before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},
		after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
		boxsep = 0mm,					%
		topsep at break=0pt,			%
		bottomsep at break=0pt,			%
		pad at break=0mm,
		pad before break=0mm,		
		pad after break=1mm,		
		bottomrule at break=0mm,
		toprule at break=0mm,		
		}}

\tcolorboxenvironment{theorem}{theoremstyle}
\tcolorboxenvironment{corollary}{theoremstyle}



\newtheoremstyle{abcd}%
  {}%
  {}%
  {\itshape}%
  {}%
  {\scshape}%
  {.}%
  {.5em}	%
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}%

\theoremstyle{abcd}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{corollary}


\tcbset{
  patternsummary/.style={
    colback=gray!2,
    colframe=gray!40,
    boxrule=0.4pt,
    arc=0mm,
    left=1mm,
    right=1mm,
    top=1mm,
    bottom=1mm
  }
}














\tcbset{qrboxstyle/.style={
		enhanced jigsaw,	%
		colback=gray!20,
		colframe=gray!40,
		arc=0mm,
		boxrule=1pt,		%
		left=1pt,
		right=1pt,
		topsep at break=1mm,			%
		top=1pt,		%
		bottom=0mm,		%
		breakable,		%
		parbox = false		%
		}}


\newcommand{\resultbox}[1]{
\begin{tcolorbox}[
	enhanced jigsaw,		%
	colback=red!5,
	colframe=red!75!black,	
	arc=0mm,
	left skip=0mm,
	right skip=0mm,	
	left=0mm,
	topsep at break=1mm,			%
	right=0mm,
	top=0mm,
	bottom=0mm,		%
	breakable,		%
	parbox = false		%
]
\emph{#1}
\end{tcolorbox}
}















\renewcommand\dbltopfraction{1} %
\renewcommand\topfraction{1} 	%
\setcounter{dbltopnumber}{8}	%
\setcounter{topnumber}{8}		%






\usepackage{adjustbox}
\def\eox{\unskip\kern 10pt{\unitlength1pt\linethickness{.4pt}$\diamondsuit${}}}   




	





\makeatletter
\DeclareRobustCommand*\uell{\mathpalette\@uell\relax}
\newcommand*\@uell[2]{
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.1ex \hbox{\kern\dimen0\unhbox1\kern\dimen0}}
}
\makeatother





\newcommand{\smallsection}[1]{\vspace{5mm}\noindent\textbf{#1.}} %
\newcommand{\introparagraph}[1]{\textbf{#1.}} %

\renewcommand{\epsilon}{\varepsilon} %
\newcommand{\set}[1]{\{#1\}}                    %
\newcommand{\setof}[2]{\{{#1}\mid{#2}\}}        %


\usepackage{mathtools}
\newcommand{\define}{\coloneqq}




\newcommand{\datarule}{{\,:\!\!-\,}} %
\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\transpose}{\intercal}	%

\newcommand{\N}{\mathbb{N}} %
\newcommand{\R}{{\mathbb{R}}} %
\newcommand{\bigO}{{\mathcal{O}}} %
\renewcommand{\O}{{\mathcal{O}}} %
\renewcommand{\P}{{\mathbb{P}}} %
\newcommand{\PP}[1]{\mathbb{P} [ #1 ]} %
\newcommand{\sql}[1]{\texttt{{#1}}}
\newcommand{\datastyle}[1]{\texttt{#1}}






    
    




\newcommand{\formattedurl}[2]{\href{#1}{\small\texttt{#2}}\xspace}







\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}
\definecolor{myred}{rgb}{1,0,0}
\definecolor{mylightblue}{rgb}{0.953, 0.957, 0.980} 	%
\definecolor{mylightblueborder}{rgb}{0.567, 0.627, 0.757} 	%
\definecolor{mylightyellow}{rgb}{0.988, 0.957, 0.863} 	%


\lstdefinestyle{codebase}{
  rulecolor=\color{mylightblueborder},
  basicstyle=\linespread{0.9}\ttfamily\small,
  columns=fullflexible,%
  breakatwhitespace=false,
  breaklines=true,
  captionpos=b,
  commentstyle=\color{mygreen},
  frame=single,
  keepspaces=true,
  numbers=none,%
  showspaces=false,
  showstringspaces=false,
  showtabs=false,
  stringstyle=\color{mymauve},
  tabsize=2,
  xleftmargin=0.5em,%
  xrightmargin=0.5em
}

\lstdefinestyle{pythoncode}{
  style=codebase,
  language=Python,
  keywordstyle=\color{blue},
  commentstyle=\color{mygreen},
  stringstyle=\color{mymauve}
}

\lstdefinestyle{sqlcode}{
  style=codebase,
  language=SQL,
  deletekeywords={...},
  classoffset=0,
  morekeywords={SELECT, DISTINCT, FROM, WHERE, AND, OR, AS, ON, HAVING,
    SUM, AVG, COUNT,
    select, distinct, from, where, and, as, on, having,
    sum, avg, count, exists, or, join, lateral, JOIN, LATERAL,
    GROUP, BY, group, by, into},
  keywordstyle=\color{blue}\bfseries,
  classoffset=1,
  morekeywords={not, in, any, all, OR, UNION, IN, ANY, ALL, NOT, EXISTS, LEFT, IS, NULL,
    is, null, x},
  keywordstyle=\color{myred},
  classoffset=2,
  morekeywords={query, block1, block2, block3, block4, qb1, qb2, qb3, qb4, subquery2},
  keywordstyle=\color{gray},
  classoffset=0
}


\lstdefinelanguage{J}{
  sensitive=true,
  alsoletter={.},
  morecomment=[l]{NB.},
  morestring=[b]',
  morekeywords={
    if.,do.,else.,elseif.,end.,
    while.,whilst.,for.,
    select.,case.,fcase.,
    try.,catch.,catchd.,throw.,
    return.,assert.,break.,continue.,
    goto.,label.
  },
  keywordstyle=\color{blue},
  ndkeywords={
    monad,dyd,dyad,
    noun,verb,adverb,conjunction,
    rank,hook,fork,cap,fit
  },
  ndkeywordstyle=\color{myred},
  commentstyle=\color{mygreen},
  stringstyle=\color{mymauve}
}

\lstdefinestyle{jcode}{
  style=codebase,
  language=J
}












\RequirePackage{scalerel}
\RequirePackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\RequirePackage{etoolbox}
\DeclareRobustCommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1, transform shape]
    \pic{orcidlogo};
\end{tikzpicture}
}{|}}}}
 




\newcommand{\equal}{\!=\!}

\let\oldin\in
\renewcommand{\in}{\!\oldin\!}
\renewcommand{\L}{\mathcal{L}}

\newcommand{\rep}{\textrm{rep}}
\newcommand{\ex}{\textrm{exp}}

\newcommand{\RA}{\textsf{RA}}
\newcommand{\NDRA}{\RA^{*}}
\newcommand{\NDRAPlain}{\RA*}
\newcommand{\NDRAA}{\RA^{*\antijoin}}

\newcommand{\Datalog}{\textsf{Datalog}}
\newcommand{\DatalogN}{\Datalog^{\neg}}
\newcommand{\DatalogND}{\Datalog^{*}}

\newcommand{\FOL}{\textsf{FOL}}
\newcommand{\DRC}{\textsf{DRC}}
\newcommand{\TRC}{\textsf{TRC}}
\newcommand{\ARC}{\textsf{ARC}}
\newcommand{\GTRC}{\textsf{G-TRC}}
\newcommand{\RC}{\textsf{RC}}
\newcommand{\NDTRC}{\TRC^{*}}
\newcommand{\NDTRCPlain}{\TRC*}

\newcommand{\SQL}{\textsf{SQL}\xspace}
\newcommand{\souffle}{\textsf{Souffl\'e}\xspace}
\newcommand{\NDSQL}{\textsf{SQL}^{*}}


\newcommand{\NRD}{\textsf{RD}^{*}}
\newcommand{\RD}{\textsf{RD}}

\newcommand{\QBE}{\textsf{QBE}}




 


\newcommand{\diagram}{\textsf{Relational Diagram}}
\newcommand{\diagrams}{\textsf{Relational Diagrams}}

\newcommand{\diagramNDnomath}{\texorpdfstring{\textsf{Relational Diagram}$^{*}$}{\textsf{Relational Diagram*}}}

\newcommand{\diagramsNDnomath}{\texorpdfstring{\textsf{Relational Diagrams}$^{*}$}{\textsf{Relational Diagrams*}}}
\newcommand{\diagramsND}{{\textsf{Relational Diagrams}^{*}}}	%














\definecolor{carfigORcolor}{HTML}{e77a30}

\newcommand{\h}[1]{\textcolor{red}{#1}} 	%
\newcommand{\hb}[1]{\textcolor{carfigORcolor}{#1}} 	%

\newcommand{\var}{\mathit{var}} 		
\newcommand{\const}{\mathit{const}} 	

\newcommand{\symb}{\bullet\;} 	

\newcommand{\antijoin}{\triangleright}

\newcommand{\tablesandattributes}{\textbf{Tables \& attributes}\xspace}
\newcommand{\constqualifications}{\textbf{Selection predicates}\xspace}
\newcommand{\joinattr}{\textbf{Join predicates}\xspace}
\newcommand{\quantifiers}{\textbf{Quantifiers}\xspace}
\newcommand{\nestingorder}{\textbf{Nesting order}\xspace}

\newcommand{\ittablesandattributes}{\emph{Tables \& attributes}\xspace}
\newcommand{\itconstqualifications}{\emph{Selection predicates}\xspace}
\newcommand{\itjoinattr}{\emph{Join predicates}\xspace}
\newcommand{\itquantifiers}{\emph{Quantifiers}\xspace}
\newcommand{\itnestingorder}{\emph{Nesting order}\xspace}

\definecolor{selPredicateColor}{HTML}{FFFFFF} 
\definecolor{selectBoxColor}{HTML}{BFBFBF}

\setlength{\fboxsep}{2pt}
\newcommand{\selPredicateBox}[1]{\fcolorbox{black}{selPredicateColor}{\textcolor{black}{#1}}}
\newcommand{\tableBox}[1]{\fcolorbox{black}{black}{\textcolor{white}{#1}}}
\newcommand{\attributeBox}[1]{\fcolorbox{black}{white}{\textcolor{black}{#1}}}
\newcommand{\selectBox}{\fcolorbox{black}{selectBoxColor}{\textcolor{white}{Q}}}


\newcommand{\E}{\mathcal{E}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\schema}{\textsf{schema}}

\newcommand{\countagg}{\textsf{count}}











\usepackage{xurl}%




\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle, fill=gray,inner sep=1.0pt] (char) {\phantom{0}};
    \node[text=white] at (char) {\textnormal{#1}};}}

\newcommand*\builtinlabel[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle, fill=white, draw, inner sep=0.4pt] (char) {\phantom{0}};
    \node[text=black] at (char) {#1};}}
















\usepackage{xparse}
\newcommand{\BraceSep}{-0.3em}  %

\NewDocumentCommand{\dgal}{sO{}m}{%
  \IfBooleanTF{#1}
    {\dgalext{#3}}%
    {\dgalx[#2]{#3}}%
}

\NewDocumentCommand{\dgalext}{m}{%
  \sbox0{%
    \mathsurround=0pt
    $\left\{\vphantom{#1}\right.\kern-\nulldelimiterspace$%
  }%
  \sbox2{\{}%
  \ifdim\ht0=\ht2
    \{\kern\BraceSep \{#1\}\kern\BraceSep\}%
  \else
    \left\{\kern\BraceSep\left\{#1\right\}\kern\BraceSep\right\}%
  \fi
}

\NewDocumentCommand{\dgalx}{om}{%
  \sbox0{\mathsurround=0pt$#1\{$}%
  \sbox2{\{}%
  \ifdim\ht0=\ht2
    \{\kern\BraceSep \{#2\}\kern\BraceSep\}%
  \else
    \mathopen{#1\{\kern\BraceSep #1\{}%
    #2%
    \mathclose{#1\}\kern\BraceSep #1\}}%
  \fi
}







\makeatletter   %

\NewDocumentCommand{\HA}{m o}{%
  \IfNoValueTF{#2}{\HA@place{#1}{#1}}%
                  {\HA@place{#2}{#1}}%
}
\newcommand{\HA@place}[2]{%
  \@ifundefined{HAseen@#1}
    {%
      \expandafter\gdef\csname HAseen@#1\endcsname{}%
      \raisebox{8mm}[0pt][0pt]{\phantomsection\label{HA:#1}}%
      {\color{purple}#2}%
    }
    {%
      \@latex@warning{Anchor `#1' declared more than once by \string\HA}%
      {\color{purple}#2}~\textcolor{red}{[Error: anchor ``#1'' defined twice]}%
    }%
}

\NewDocumentCommand{\HL}{m o}{%
  \IfNoValueTF{#2}{\HL@to{#1}{#1}}%
                  {\HL@to{#2}{#1}}%
}
\newcommand{\HL@to}[2]{%
  \@ifundefined{r@HA:#1}%
    {\textcolor{red}{[Error: link ``#1'' has no anchor]}}%
    {\hyperref[HA:#1]{#2}}%
}

\makeatother







